SynDiffix: More accurate synthetic structured data

This paper introduces SynDiffix, a mechanism for generating statistically accurate, anonymous synthetic data for structured data. Recent open source and commercial systems use Generative Adversarial Networks or Transformed Auto Encoders to synthesize data, and achieve anonymity through overfitting-avoidance. By contrast, SynDiffix exploits traditional mechanisms of aggregation, noise addition, and suppression among others. Compared to CTGAN, ML models generated from SynDiffix are twice as accurate, marginal and column pairs data quality is one to two orders of magnitude more accurate, and execution time is two orders of magnitude faster. Compared to the best commercial product we measured (MostlyAI), ML model accuracy is comparable, marginal and pairs accuracy is 5 to 10 times better, and execution time is an order of magnitude faster. Similar to the other approaches, SynDiffix anonymization is very strong. This paper describes SynDiffix and compares its performance with other popular open source and commercial systems.

==> attacks-table.tex <==
\section{Table of Attacks}

Table \ref{tab:sd-attacks} lists all the attacks that have been analyzed for Diffix, and could apply to \sd.

% The following are here because otherwise the spacing is messed up in the table

%\begin{attack} \label{atk:one_two_poss} \end{attack}





% end labels

\begin{table}
\begin{center}
\begin{small}
\begin{tabular}{llll}
\toprule
   Attack &   &   Cite &   Section \\
\midrule
   \vspace{-1.7ex}
   \begin{attack} \label{atk:simpdiff} \end{attack}  &
   Simple difference &  \cite{diffix-aspen} &  sec 7, fig 7 \\
   
   \vspace{-1.7ex}
   \begin{attack} \label{atk:one_two_poss} \end{attack} &
   Knowledge-based (noise) &  \cite{diffix-aspen} &  sec 7, fig 8 \\
   &  &  \cite{francis2022diffix} &  sec 5.6 \\

   \vspace{-1.7ex}
   \begin{attack} \label{atk:simp_avg} \end{attack} &
   Simple averaging &  \cite{diffixBirch} &  sec 2 \\

   \vspace{-1.7ex}
   \begin{attack} \label{atk:att_inspect} \end{attack} &
   Attribute value inspection &  \cite{francis2022diffix} &  sec 5.4 \\

   \vspace{-1.7ex}
   \begin{attack} \label{atk:unique-infer} \end{attack} &
   Unique inference &  \cite{francis2022diffix} &  sec 5.5 \\

   \vspace{-1.7ex}
   \begin{attack} \label{atk:know-supp} \end{attack} &
   Knowledge-based (suppression) &  \cite{francis2022diffix} &  sec 5.7 \\

   \vspace{-1.7ex}
   \begin{attack} \label{atk:diff1} \end{attack} &
   Difference, one victim &  \cite{francis2022diffix} &  sec 5.12 \\

\bottomrule
\end{tabular}
\end{small}
\end{center}
  \caption{List of attacks that apply to \sd}
  \label{tab:sd-attacks}
\end{table}

\subsection{Attacks that can be run}

Attack \ref{atk:simpdiff} assumes a successful difference attack, and confirms the amount of noise needed to have adequate PI. With \sdx, this can only happen when one user changes from one epoch to the next.

Attack \ref{atk:one_two_poss} is where attacker knows that one of two possible counts exists, and is also used to calibrate noise.

Attack \ref{atk:simp_avg} (simple repeat of queries) does not work because of sticky noise.

Attack \ref{atk:att_inspect} behaves similar. Note that one must ensure that we don't have a single individual masquerading as multiple individuals (one person with multiple cell phones), or a tight group of individuals (a family). Strongly suggest removing PII.

Attack \ref{atk:unique-infer} (unique infer ... value of $N-k$ columns infers remaining $k$ columns) requires checks if the user is worried about it.

Attack \ref{atk:diff1} should work similar to the attack described in Elm 5.12 (probably a bit less effective). We don't have suppressed bucket merging.

Attack \ref{atk:know-supp} (knowledge-based suppression) does have some PI/PR scores inside the risk zone. Attack is outside of risk zone at mean thresh of 10. But special data conditions and attacker knowledge make this attack extremely rare.

\subsection{Attacks that cannot be run}

Table \ref{tab:sd-non-attacks} lists all the attacks that have been analyzed for Diffix, and but cannot be applied to \sd because the API does not allow them.

\begin{table}
\begin{center}
\begin{small}
\begin{tabular}{llll}
\toprule
   & Attack &   Cite &   Section \\
\midrule
   \begin{attack} \label{atk:split_avg} \end{attack} &
   Split averaging &  \cite{diffixBirch} &  sec 5.2.1 \\

   \begin{attack} \label{atk:chaff} \end{attack} &
   Chaff conditions &  \cite{diffixBirch} &  sec 5.2.4 \\

\bottomrule
\end{tabular}
\end{small}
\end{center}
  \caption{List of attacks that cannot be run against \sd because the API doesn't allow it.
  }
  \label{tab:sd-non-attacks}
\end{table}

Attack~\ref{atk:split_avg} requires \mytt{AND NOT}.

==> criteria.tex <==
\section{Anonymity and performance criteria}
\label{sec:criteria}

Maybe some discussion of data augmentation versus model quality versus descriptive analytics.

Perhaps mention that we are interested in performance for both descriptive and ML use cases.

Say that our criteria for anonymity is adapted from (hmmm, not sure. maybe we don't need this section?)

Mention why we don't used differential privacy as a measure.
